Determinacy with Priorities up to Clocks

In Milner's seminal book on communication and concurrency introducing CCS, a process algebra inherently non-deterministic, chapter 11 was completely devoted to introduce the notion of determinacy and confluence in order to identify a subcalculus of CCS in which all definable agents are confluent. At the same time, or shortly later, determinate semantics were given for programming languages that reconcile concurrency and determinacy, such as Esterel by Berry and Gonthier, or SL by Boussinot and de Simone. These dedicated semantics do not easily map to Milner's confluence theory for CCS, which is unable to express causality and shared memory multi-threading with reaction to absence in a compositional way. We present an extension of CCS with priority-guarded actions and clocks, and we exploit the added expressiveness to enrich Milner's original notion of confluence by the new concept of coherence which permits us to encode, in a compositional fashion, synchronous programming languages such as Esterel.

==> eptcsdata.tex <==
\providecommand{\firstpage}{79}
\providecommand{\publicationstatus}{Lorenzo Gheri \& Kirstin Peters (Eds.): 17th International\\ Workshop on Programming Language Approaches to Concurrency\\ and Communication-cEntric Software 2026 (PLACES 2026)\\
EPTCS 444, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.444.8}{10.4204/EPTCS.444.8}}
\pdfoutput=1

